GStarX: Explaining Graph Neural Networks with Structure-Aware Cooperative Games

Explaining machine learning models is an important and increasingly popular area of research interest. The Shapley value from game theory has been proposed as a prime approach to compute feature importance towards model predictions on images, text, tabular data, and recently graph neural networks (GNNs) on graphs. In this work, we revisit the appropriateness of the Shapley value for GNN explanation, where the task is to identify the most important subgraph and constituent nodes for GNN predictions. We claim that the Shapley value is a non-ideal choice for graph data because it is by definition not structure-aware. We propose a Graph Structure-aware eXplanation (GStarX) method to leverage the critical graph structure information to improve the explanation. Specifically, we define a scoring function based on a new structure-aware value from the cooperative game theory proposed by Hamiache and Navarro (HN). When used to score node importance, the HN value utilizes graph structures to attribute cooperation surplus between neighbor nodes, resembling message passing in GNNs, so that node importance scores reflect not only the node feature importance, but also the node structural roles. We demonstrate that GStarX produces qualitatively more intuitive explanations, and quantitatively improves explanation fidelity over strong baselines on chemical graph property prediction and text graph sentiment classification.

==> sections/analysis.tex <==
In this section, we analyze the good properties of the HN value, show their advantage over the Shapley value for cooperative game with communication structures, and show these properties matches the intuition of graph machine learning models.

We first compare these two values by checking their values on unanimity games.

\subsection{Unanimity Games}
The unanimity game, $(N, v_T)$, is a special type of games defined on a coalition $T \subseteq N$. For all $S \subseteq N$,
\begin{equation} \label{eq:unanimity_game}
    v_{T}(S) = 
    \begin{cases}
    1 & \text{if } T \subseteq S \\
    0 & \text{if } T \nsubseteq S
    \end{cases}
\end{equation}

According to Lemma 3 in Shapley, any game with a finite number of players can be written as a linear combination of unanimity games \yrcite{shapley}:
\begin{equation} \label{eq:unanimity_game_linear_comb}
    v = \sum_{T \subseteq N} c_{T} (v) v_{T}
\end{equation}

The unanimity games thus work as a basis for generating the whole space of games. They are usually the first example to study for a newly proposed value.



Graphormer
\cite{graphormer}


popular GNN architectures, , GIN \cite{gin}, and GAT \cite{gat}


% Note that our SubgraphX treats the GNNs as black boxes during the explanation stage and only needs to access the inputs and outputs. Hence, our proposed SubgraphX can be applied to a general family of GNN models, including but not limited to GCNs (Kipf & Welling, 2017), GATs (Velicˇkovic ́ et al., 2018), GINs (Xu et al., 2019), and Line-Graph NNs (Chen et al., 2018b).

\subsection{Model-Agnostic Explanation}
Our method is model-agnostic, we thus further investigate its performance on more GNN architectures, GIN and GAT. We follow \citet{subgraphx} to train GIN on \mutag and GAT on \sst. Since the full evaluation of the \sst dataset can take more than 24 hours to finish for SubgraphX, we only consider a subset of 50 nodes.
\begin{table*}[ht]
\center
\caption{Harmonic Fidelity}
\begin{tabular}{@{}llllll@{}}
\toprule
\multicolumn{1}{l}{Dataset} & \multicolumn{1}{l}{GNNExplainer} & PGExplainer & SubgraphX & Ours  \\ \midrule
\mutag &&&&  \\
\bbbp &&&&   \\ 
\sst &&&&    \\ 
\bamotif &&&&  \\ 
\bottomrule
\end{tabular}
\label{tab:harmonic_fidelity}
\end{table*}


\subsection{Efficiency Comparison }
Our method is model-agnostic, we thus further investigate its performance on more GNN architectures, GIN and GAT. We follow \citet{subgraphx} to train GIN on \mutag and GAT on \sst. Since the full evaluation of the \sst dataset can take more than 24 hours to finish for SubgraphX, we only consider a subset of 50 nodes.
\begin{table*}[ht]
\center
\caption{Efficiency}
\begin{tabular}{@{}llllll@{}}
\toprule
\multicolumn{1}{l}{Dataset} & \multicolumn{1}{l}{GNNExplainer} & PGExplainer & SubgraphX & Ours  \\ \midrule
\bbbp &&&&   \\ 
\sst &&&&    \\ 
\bottomrule
\end{tabular}
\label{tab:harmonic_fidelity}
\end{table*}
